Scalable Neural Network Kernels

We introduce the concept of scalable neural network kernels (SNNKs), the replacements of regular feedforward layers (FFLs), capable of approximating the latter, but with favorable computational properties. SNNKs effectively disentangle the inputs from the parameters of the neural network in the FFL, only to connect them in the final computation via the dot-product kernel. They are also strictly more expressive, as allowing to model complicated relationships beyond the functions of the dot-products of parameter-input vectors. We also introduce the neural network bundling process that applies SNNKs to compactify deep neural network architectures, resulting in additional compression gains. In its extreme version, it leads to the fully bundled network whose optimal parameters can be expressed via explicit formulae for several loss functions (e.g. mean squared error), opening a possibility to bypass backpropagation. As a by-product of our analysis, we introduce the mechanism of the universal random features (or URFs), applied to instantiate several SNNK variants, and interesting on its own in the context of scalable kernel methods. We provide rigorous theoretical analysis of all these concepts as well as an extensive empirical evaluation, ranging from point-wise kernel estimation to Transformers' fine-tuning with novel adapter layers inspired by SNNKs. Our mechanism provides up to 5x reduction in the number of trainable parameters, while maintaining competitive accuracy.

==> fourier_transforms.tex <==
\section{Fourier Transforms of some commonly used activation functions}
In this section we compute the Fourier Transform of some well-known activation functions. 

\subsection{GELU}
The Gelu activation is given by $f(x)= x \Phi(x)$, where $\Phi$ is the standard Gaussian cumulative distribution function. Now the Fourier transform of 
$FT[xf(x)] = i\frac{d\hat{f}(k)}{dk}$. The proof is as follows: 
\begin{equation}~\label{eqn:ft_formula}
    \begin{split}
        FT[xf(x)]  & = \int xf(x)e^{-ikx}dx \\
                    & = \int f(x) i(\frac{d}{dk}e^{-ikx})dx \\
                    & = i\frac{d}{dk}\int f(x)e^{-ikx}dx \\
                    & = i\frac{d}{dk} \hat{f}(k) \\
    \end{split}
\end{equation}

So in our case, 
\begin{equation} \label{gelu_ft}
\begin{split}
FT[x\Phi(x)] & = i\frac{d\hat{\Phi}(k))}{dk} \\
 & = \textcolor{red}{-ike^{-k^2/2}}
\end{split}
\end{equation}

\subsection{Sigmoid}
To compute the FT of sigmoid, one proceeds as follows : 
\begin{equation} \label{sigmoid_ft}
FT[\frac{e^{x}}{1+e^{x}}]  = \int_{0}^{\infty} \frac{e^{x(1-ik)}}{1+e^x}dx+ \int_{-\infty}^{0} \frac{e^{x(1-ik)}}{1+e^x}dx
\end{equation}
We first solve the first integral, we divide both the numerator and denominator by $e^x$, i.e.
\begin{equation}
    \frac{e^{x(1-ik)}}{1+e^x} = \frac{e^{x(1-ik)}}{e^{x}(1+e^{-x})} = \frac{e^{-ixk}}{1+e^{-x}}
\end{equation}
Using the Taylor series expansion for 
\begin{equation}
    \frac{1}{1+e^{-x}} = \Sigma_{n=0}^{\infty} (-1)^ne^{-nx}
\end{equation}
Thus the integral can be computed as 
\begin{equation}
    \Sigma_{n=0}^{\infty} (-1)^n\int_{0}^{\infty} e^{x(n+ik)}dx = \Sigma_{n=0}^{\infty}(-1)^{n}\frac{1}{n+ik} := \Phi(-1,1, ik)
\end{equation}
where $\Phi$ in this case is the generalized Lerch Phi function. 
To compute the other half of the integral, follow the above steps but in this case, use :
\begin{equation}
    \frac{1}{1+e^{x}} = \Sigma_{n=0}^{\infty}(-1)^n e^{nx}
\end{equation}
Thus the integral becomes 
\begin{equation}
    \Sigma_{n=0}^{\infty} (-1)^n\int_{-\infty}^{0} e^{x(1 -ik + n)}dx = \Sigma_{n=0}^{\infty}(-1)^{n}\frac{1}{1-ik+n} := \Phi(-1,1, 1-ik)
\end{equation}
Thus the entire integral becomes 
$\Phi(-1,1, 1-ik) + \Phi(-1,1, ik) $. Using special values and using the properties of $\Phi$-function the above sum boils down to $\frac{1}{2} i \pi  \tanh \left(\frac{\pi  k}{2}\right)-\frac{1}{2} i \pi  \coth \left(\frac{\pi  k}{2}\right)$ or more simply $-i \pi\  \text{csch}(\pi  k)$. Note that this integral only truly exists in a distributional sense where where csch is understood in the sense of the principal value. (cite complex analysis text book like Stein or Rudin)

\subsection{Swish}
The Swish activation function is given by $S(x) = \frac{x}{1+e^{-\beta x}}$. Thus 
\begin{equation}\label{swish_ft}
\begin{split}
 FT[S](k) & = i\frac{d}{dk}\Bigl(\frac{1}{1+e^{-\beta k}}\Bigr) \\
 & = i\frac{\beta e^{-\beta k}}{(1+e^{-\beta k})^2}
\end{split}
\end{equation}

\subsection{Tanh}
Similar to the computation above, we do algebraic manipulations to arrive at the FT, however one should note that the integral does not exist in the sense of a classical Riemann integral. Using the fact $\frac{d}{dt}\tanh(t) = \text{sech}^2(t)$. Thus $ikFT\left[ \tanh(t)\right](k) = FT\left[ \text{sech}^2(t)\right](k)$. Using contour integral, one gets 
\begin{equation}
FT\left[ \text{sech}^2(t)\right](k) = \int_{-\infty}^\infty dt\, e^{-ik t}\, \text{sech}^2(t) = \pi k \, \text{csch}\left(\frac{\pi k}{2} \right)
\end{equation}
Thus $FT\left[ \text{tanh}(t)\right](k) = -i \, \pi \, \mathcal{P}\, \text{csch}\left(\frac{\pi k}{2} \right)$, where $\mathcal{P}$ is the Cauchy principal value.


The other way to compute tanh is via the following~\citep{inf-kernel} : \\
$2/\sqrt{\pi}\text{tanh}(x) \sim \text{erf}$ when $|x|<.5$. This follows from the fact the Taylor series for both of the functions are the same up to the $4$th order.


\subsection{Sine}
Sine activation was used in the~\citep{sitzmann2019siren}. This is well-known and is given by : 
\begin{equation}
    FT[sin(x)] = \frac{i}{2}[\delta(k+\frac{1}{2\pi}) - \delta(k-\frac{1}{2\pi})] 
\end{equation}
Note unlike the cosine function, the Fourier transform is imaginary which is the case for odd functions.

\subsection{Relu}
The ReLu is not a positive definite kernel so Boechner's theorem does not hold. However the trick to approximate a Fourier Transform for this function is to consider a smoothed version of Relu that decays exponentially faster at $\infty$. This trick is employed in~\citep{pmlr-v125-bresler20a}. (Sorry I am missing something, I believe the arc cosine should come out of this. Mistake in my calculations )

\section{Creating Good Fourier Transforms}
This is a simple generalization of the methods presented in~\citep{pmlr-v125-bresler20a}. Most of the Fourier integrals that we are concerned about are complex functions. To get real Fourier transforms, we follow these steps. First note that $FT[f]$ is real iff $f(x) = \overline{f(-x)}$. Thus one can obtain real Fourier integrals if one simply approximate a continuous function by an even function. The basic idea is to to choose a function $\phi$ with the following properties 
\begin{enumerate}
    \item $\phi \in C^{\infty}(-\epsilon, \epsilon)$, for $\epsilon$ small enough $\epsilon$
    \item $\phi$ is even
    \item Partition of unity, i.e. $\int \phi = 1$
    \item Moreover, one can take $x\phi' < 0$
One can prove that by suitably scaling $\epsilon$, $\phi * f \rightarrow f$. Such $\phi$ are dense in $C(-\epsilon, \epsilon)$. 
%It is a simple exercise to check that convolution of 2 even functions is even. 
TODO : write the proof (see Theorem 11.21 and lemma 11.21 for the proof in \url{https://mathweb.ucsd.edu/~bdriver/231-02-03/Lecture_Notes/Chapter%2011-%20Convolutions%20and%20Approximations.pdf} However, we note that a good approximation by an even function may not exist but if one can construct the Fourier transform of the $\phi * f$. A simple recipe to construct a sequence $\{\phi\}$ is to start with $f \in L^1 $ and $\phi_n := t^{-n} f(x/t^{n})$
\end{enumerate}

\section{Using Polynomial Kernels for Brute Force Construction of Random Features}
\cite{pmlr-v22-kar12} constructs random features for kernels of the form $\mathrm{K}(\vx,\vy) = f(\vx\vy^\top)$, where $f$ has a power series expansion of the form $f:= \sum a_n x^n$, and $a_n \geq 0$. This can be easily extended to the case where $f$ does not necessarily have positive Taylor coefficients. Write $f$ as $f:= f_1 - f_2$, where $f_1$ and $f_2$ have positive coefficients, and $\mathrm{K}(\vx,\vy) = \mathrm{K}_1(\vx,\vy) - \mathrm{K}_2(\vx,\vy)$. Each $\mathrm{K}_i$ admits a random feature mechanism $\Phi_i$ and thus 
$\mathrm{K}(\vx,\vy) \sim [\Phi_1(\vx) | \Phi_2(\vx)] [\Phi_1(\vy) | -\Phi_2(\vy)]^{\top} $ where $|$ refers to concatenation of 2 vectors along their columns. The approximation error can trivially be bounded by the sum of the approximation errors for each factor. We refer to this construction as the brute force variant. 
% and assume that both $f_1$ and $f_2$ converge (I am fairly sure that this is always the case. Will write out a proof)
\subsection{Extending polynomial kernels to tanh}~\label{sec:tanh_kernel}
Tanh is an odd function so $a_n = 0$, if n is even. Moreover, the non-zero terms alternate in sign, i.e. 
\[
    a_n 
\begin{cases}
    > 0,& \text{if } n\equiv 1 (\text{mod} \  4)\\
    < 0,              & \text{if } n\equiv 3 (\text{mod} \ 4) \\
    = 0  & \text{otherwise}
\end{cases}
\]
Splitting it up in 2 power series with the positive and negative terms produces extremely sparse kernels $\Phi_i$, and this is due to the external measure used in~\citep{pmlr-v22-kar12}. Even with rejection sampling, i.e. essentially sampling only odd terms still produces sparse kernels. This becomes a bottleneck in the pooler experiments where most of the accuracies are contributed by the pretrained features and applying a sparse kernel distorts them. We use the same random Rademacher matrices for construction of both $\mathrm{K}_1$ and $\mathrm{K}_2$ as it reduces the variance~\citep{choromanski2022hybrid}. 

Table~\ref{tab:tanh_res} shows some results using the above kernel for the pooler experiments. The results are considerably worse for larger datasets. This negative results show the need for developing novel techniques discussed in this paper. 

==> theory.tex <==
\section{Theoretical results}
\label{sec:theory}
